Direct optimization of F-measure for retrieval-based personal question answering

Recent advances in spoken language technologies and the introduction of many customer facing products, have given rise to a wide customer reliance on smart personal assistants for many of their daily tasks. In this paper, we present a system to reduce users' cognitive load by extending personal assistants with long-term personal memory where users can store and retrieve by voice, arbitrary pieces of information. The problem is framed as a neural retrieval based question answering system where answers are selected from previously stored user memories. We propose to directly optimize the end-to-end retrieval performance, measured by the F1-score, using reinforcement learning, leading to better performance on our experimental test set(s).

==> figure.tex <==
% Below is an example of how to insert images. Delete the ``\vspace'' line,
% uncomment the preceding line ``\centerline...'' and replace ``imageX.ps''
% with a suitable PostScript file name.
% -------------------------------------------------------------------------
\begin{figure}[htb]

\begin{minipage}[b]{1.0\linewidth}
  \centering
  \centerline{\includegraphics[width=8.5cm]{img/image1}}
%  \vspace{2.0cm}
  \centerline{(a) Result 1}\medskip
\end{minipage}
%
\begin{minipage}[b]{.48\linewidth}
  \centering
  \centerline{\includegraphics[width=4.0cm]{img/image3}}
%  \vspace{1.5cm}
  \centerline{(b) Results 3}\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.48\linewidth}
  \centering
  \centerline{\includegraphics[width=4.0cm]{img/image4}}
%  \vspace{1.5cm}
  \centerline{(c) Result 4}\medskip
\end{minipage}
%
\caption{Example of placing a figure with experimental results.}
\label{fig:res}
%
\end{figure}


==> model.tex <==
\section{END-TO-END SYSTEM}
\label{sec:model}

We experiment with both probabilistic and deterministic models for the purpose of determining relevant memories for a given query. Given a query $q$, and its corresponding set of memories $M_q = \{m_1, ..., m_{|M_q|}\}$, we denote the relevant queries by $R_q \subseteq M_q$.

\subsection{Model Features}

We use word embeddings as input features for our models. For our baseline models, we use pre-trained $\mathtt{fasttxt}$ word embeddings. These word vectors were trained using the CBOW model with positional-weighting (for the context vectors), and incorporate phrase representations in form of word n-gram tokens (also, subword knowledge in the form of bag of character n-gram vectors - we do not use this version), which are also learnt from the data. These word vectors were trained on Wikipedia data from $2017$, news datasets from \texttt{statmt.org} from $2007-2016$ as well as the UMBC corpus \cite{han2013umbc_ebiquity}. We also experiment with character-aware word embeddings that are trained using task-specific criteria. These character-aware word embeddings with word embeddings, and are not used standalone.

For a given word $w = (c_1, ..., c_{|w|})$, we represent its word vector as $\mbv_w \in \mathbb{R}^d$, where $d$ is the dimension of the word vector. For a given query $q = (w_1, ..., w_{|q|})$, we define its feature vector to be the matrix of word embeddings

\begin{equation*}
E_q = [\mbv_{w_1}, ..., \mbv_{w_{|q|}}] \in \mathbb{R}^{|q| \times d}.
\end{equation*}

where $|q|$ denotes the length of the query in words. We use similar terminology for the memory vectors as well, denoted by $E_{m_i} \in \mathbb{R}^{|m_i| \times d}$, where $|m_i|$ denotes the length of the memory in words.


\subsection{Model Structure}

In this section, we describe the complete array of models used in our information retrieval system.

\subsubsection{Baselines - $\mathtt{cosine*}$}

Our baseline models involve no learning and are a purely deterministic system. We use a \acrfull{BOW} model together with a Cosine similarity metric, which determines the probability of a relevant memory. More specifically, this model consumes the query feature vector, $E_q$ and the memory feature vectors $\{E_{m_1}, ..., E_{m_{|M_q|}}\}$, and produces a pair-wise relevance score as

\begin{equation*}
p(m_i \in R_q | q) = \mathtt{CosineSimilarity}(\mathtt{agg}(E_q), \mathtt{agg}(E_{m_i}))
\end{equation*}

where $\mathtt{agg} : \mathbb{R}^{l \times d} \mapsto \mathbb{R}^{d}$ is an aggregator function that produces a fixed-length vector from variable length feature vectors, by aggregating along the length dimension. We experiment with different aggregator functions in our baseline, including the $\mathtt{max}$ (max of word vectors across each dimension), $\mathtt{sum}$ (sum of word vectors) and $\mathtt{avg}$ (mean of word vectors) aggregators. We denote this model as $\mathtt{cosine}$ (and append the name of the aggregator function for identification purposes).

We also experiment with the coattention encoder (cite needed) as an aggreagate function for our cosine similarity models. For a given query-memory pair $q$ and $m$, we first compute the affinity matrix as

\begin{equation*}
  L = E_m  E_q^{\top} \in \mathbb{R}^{|m| \times |q|}
\end{equation*}

The attention weights for the memory attending to the query are computed by normalizing the affinity matrix row-wise as

\begin{equation*}
  A^q = \text{softmax}(L) \in \mathbb{R}^{|m| \times |q|}
\end{equation*}

and similarly, the attention weights for the query attending to each word in the memory is computed by normalizing the affinity-matrix column-wise as

\begin{equation*}
  A^m = \text{softmax}(L^{\top}) \in \mathbb{R}^{|q| \times |m|}
\end{equation*}

The attention contexts are then computed as

\begin{equation*}
  C^q = A_q^{\top}E^m \hspace{2px} \in \mathbb{R}^{|q| \times d} \text{ and } \hspace{2px} C^m = A_m^{\top}E^q \in \mathbb{R}^{|m| \times d}
\end{equation*}

These attention contexts are used as the feature vectors and the $\mathtt{coatt}$ aggregator is then defined as the average of these contexts, i.e.

\begin{align*}
  \mathtt{coatt} &: E_q \mapsto \mathtt{avg}(C^q) \\
  &: E_m \mapsto \mathtt{avg}(C^m)
\end{align*}
% \mathtt{coatt} : E_q \mapsto avg(C^q) \text{ and } E_m \mapsto avg(C^m)

\subsubsection{$\mathtt{CharEmbedding}$ and $\mathtt{ChrWrdFF}$}

We also train character-aware word embeddings for the task-specific loss (see below). We use a convolutional model with multiple filters of varying width, to capture long-range sub-word information effectively.

For a given word $w = (c_1, ..., c_{|w|})$, let $\mbC_w \in \mathbb{R}^{|w| \times d}$ be the character-level representation of $w$, where $d$ is the dimension of the character embeddings (not necessarily the same as word vector dimensionality, abuse of notation). We apply a convolution between $\mbC_w$ and a kernel $\mbK_i \in \mathbb{R}^{k \times d \times n}$ of width $k$ and $n$ output channels, followed by non-linearity and max-pool layers.

\begin{align*}
  y_i &= \mbC_w \ast \mbK_i  + b_i \in \mathbb{R}^{\hat{|w|} \times n} \\
  y_i &= \mathtt{maxpool}(\mathtt{relu}(y_i)) \in \mathbb{R}^n
\end{align*}

We do this for $f$ kernels of varying width and concatenate the output of these $f$ convolutions before applying a final linear layer to produce embeddings of dimension $d$.

\begin{align*}
  y &= \mathtt{concat}(y_1, ..., y_f) \in \mathbb{R}^{f\cdot n} \\
  \mby_w &= \mathtt{Linear}(y) \in \mathbb{R}^{d}
\end{align*}

The combined character-aware and pre-trained word embeddings is given by $\mbu_w = \mathtt{concat}(\mbv_w, \mby_w)$. We refer to this character-aware embedding model as $\mathtt{CharEmbedding}$ in our results.

We report a baseline model using the combined word vectors $\mbu_w$. Given the query and memory feature tensors $E_q$ and $E_m$ (using the concatenated word vectors $\mbu_w$), we aggreagate them by taking the maximum column-wise to produce $d$-dimensional vectors and use compute a Hadamard product between these two vectors to get the joint activations for each query-memory pair.

\begin{align*}
  \hat{E_q} &= \mathtt{max}(E_q) \in \mathbb{R}^d \text{ and } \hat{E_m} = \mathtt{max}(E_m) \in \mathbb{R}^d \\
  y&= \hat{E_q} \odot \hat{E_m} \in \mathbb{R}^d \\
  y&= \mathtt{Linear}(y) \in \mathbb{R}^{\hat{d}} \\
  y&= \mathtt{dropout}(\mathtt{relu}(y)) \\
  \mathtt{logits} &= \mathtt{softmax(y)} \in \mathbold{R}^2
\end{align*}

We apply a linear layer, followed by $\mathtt{relu}$ non-linearity and dropout to compute the output score for this query-memory pair. We refer to this model as $\mathtt{ChrWrdFF}$, and use it as a baseline probabilistic model.
\subsubsection{$\mathtt{SARD}$ and $\mathtt{SARDCH}$}

Our $\mathtt{SARD}$ model is a neural attention model, similar to the architecture described in (cite needed). This architecture is composed of a stack of various neural layers; a highway layer (cite needed), followed by a multi-head self-attention layer with residual connections, position-wise feed-forward layers and layer normalization (the $\mathtt{transformer\_block}$ from ``Attention is All You Need''), followed by fully-connected layers and the output layer.

TODO: Add figure and eqn's describing attention

The $\mathtt{SARDCH}$ model is identical to the $\mathtt{SARD}$ model, but uses the concatenated embedddings produced by the $\mathtt{CharEmbedding}$ model, which is trained together with this architecture end-to-end.


\subsubsection{$\mathtt{TEFF}$ and $\mathtt{TEFFCH}$}

The $\mathtt{TEFF}$ model is a model comprised of two fully-connected layers of the form

\begin{align*}
  y &= \mathtt{Linear}(E_q) \in \mathbb{R}^{|q| \times h} \\
  y &= \mathtt{dropout}(\mathtt{relu}(y)) \\
\end{align*}

and similarly applied to $E_m$. The two feature tensors are then aggregated along the first dimension to produce $h$-dimensional representations of the query and memory, $u$ and $v$ respectively. The joint activation and the logits are computed as

\begin{align*}
  y &= \mathtt{concat}(u, v, |u-v|, u\odot v) \\
  \mathtt{logits} &= \mathtt{softmax}(\mathtt{dropout}(y)) \in \mathbb{R}^2 \\
\end{align*}

The $\mathtt{TEFFCH}$ model includes the $\mathtt{CharEmbedding}$ module together with the $\mathtt{TEFF}$ architecture, and again is jointly trained.


==> relatedworks.tex <==
%\section{Related Works}
\label{sec:rework}



==> type_style.tex <==
\section{TYPE-STYLE AND FONTS}
\label{sec:typestyle}

To achieve the best rendering both in printed proceedings and electronic proceedings, we
strongly encourage you to use Times-Roman font.  In addition, this will give
the proceedings a more uniform look.  Use a font that is no smaller than nine
point type throughout the paper, including figure captions.

In nine point type font, capital letters are 2 mm high.  {\bf If you use the
smallest point size, there should be no more than 3.2 lines/cm (8 lines/inch)
vertically.}  This is a minimum spacing; 2.75 lines/cm (7 lines/inch) will make
the paper much more readable.  Larger type sizes require correspondingly larger
vertical spacing.  Please do not double-space your paper.  TrueType or
Postscript Type 1 fonts are preferred.

The first paragraph in each section should not be indented, but all the
following paragraphs within the section should be indented as these paragraphs
demonstrate.

